Improved Battery State Estimation Under Parameter Uncertainty Caused by Aging Using Expansion Measurements

Accurate tracking of the internal electrochemical states of lithium-ion battery during cycling enables advanced battery management systems to operate the battery safely and maintain high performance while minimizing battery degradation. To this end, techniques based on voltage measurement have shown promise for estimating the lithium surface concentration of active material particles, which is an important state for avoiding aging mechanisms such as lithium plating. However, methods relying on voltage often lead to large estimation errors when the model parameters change during aging. In this paper, we utilize the in-situ measurement of the battery expansion to augment the voltage and develop an observer to estimate the lithium surface concentration distribution in each electrode particle. We demonstrate that the addition of the expansion signal enables us to correct the negative electrode concentration states in addition to the positive electrode. As a result, compared to a voltage only observer, the proposed observer can successfully recover the surface concentration when the electrodes' stoichiometric window changes, which is a common occurrence under aging by loss of lithium inventory. With a 5% shift in the electrodes' stoichiometric window, the results indicate a reduction in state estimation error for the negative electrode surface concentration. Under this simulated aged condition, the voltage based observer had 9.3% error as compared to the proposed voltage and expansion observer which had 0.1% error in negative electrode surface concentration.

==> Extra/Peyman_model.tex <==
\section{Model Development}
\label{Model}
\subsection{Electrochemical Model}
\begin{figure}[!t]
	\centering
	{\includegraphics[width=1\columnwidth,trim = 0in 0in 0.0in 0in,clip=true]{figures/multiSPMe_v2.pdf}}
	\caption{The schematics of the Multiparticle electrochemical and mechanical model.}
	\label{fig:2}
\end{figure}
The electrochemical model in this section is primary based on the well known Doyle Fuller Newman (DFN) model. As mentioned in the introduction, the distribution of particle size for the graphite electrode is considered here. A model for electrodes with multiple materials has been proposed in \cite{albertus2009experiments}. The treatment of multiple particle sizes is similar to models with multiple materials, with only difference being the fact that instead of multiple materials there are multiple particle sizes of the same material. The model schematics is shown in \cref{fig:2}. For generality the particle size distribution is considered for both positive and negative electrodes in the model description below, although in practice we only considered a particle distribution in the negative electrode.
\subsubsection{Full order model}
The multiparticle DFN (MP-DFN) model is presented here. The main difference in MP-DFN model is that at each point in the $x$ direction instead of the single particle configuration, there are multiple particles with a size distribution. The particle size distribution is the same along the length of the electrode. In the following equations the symbol $(*)$ is a place holder for either positive $(p)$ or negative $(n)$ electrodes. The number of particle sizes is denoted by $N_*^R$. The particle $(i)$ represents the particles with size $R_{p,i}^*$. The lithium concentration, $(c_{s,i})$, for each particle $(i)$ is given by the following solid diffusion equations
\begin{flalign}
\label{diff1}
\frac{\partial c_{s,i}^*}{\partial t}(x,r,t)=\frac{1}{r^2}\frac{1}{\partial r}\left[D_{s,i}^*r^2\frac{\partial c_{s,i}^*}{\partial r}(x,r,t)\right],\\
\frac{\partial c_{s,i}^*}{\partial r}(x,0,t)=0,\\
D_{s,i}^*\frac{\partial c_{s,i}^*}{\partial r}(x,R_{p,i}^*,t)=-j_i^*(x,t),
\end{flalign}
where $j_i$ is the pore wall flux between electrolyte and the solid, and $D_s$ is the solid state diffusion coefficient. The Butler-Volmer equation is given by
\begin{flalign}
\label{bv2}
j_i^*(x,t) = \frac{i_{0,i}^*(x,t)}{F}\left(e^{\frac{\alpha_a F}{RT}\eta_i^*(x,t)}-e^{\frac{-\alpha_c F}{RT}\eta_i^*(x,t)}\right), \\   
i_{0,i}^*(x,t) = k_{0}^*({c_e}(x,t))^{\alpha_a}(c_{s,max,i}^*-c_{se,i}^*(x,t))^{\alpha_a}(c_{se,i}^*(x,t))^{\alpha_c}, 
\end{flalign}
where $c_{se,i}^*(x,t)=c_{s,i}^*(x,R_{p,i}^*,t)$ is the concentration at the surface of the particle, the $k_0$ is the reaction rate constant, the ($\alpha_a, \alpha_c$) are the charge transfer coefficients, and $ \eta_i^*(x,t)$ is the surface overpotential given by
\begin{flalign}
\label{eta1}
\eta_i^*(x,t) = \Phi_1(x,t)-\Phi_2(x,t)-U_*(c_{se,i}^*(x,t))-V_{f,i}^*(x,t),
\end{flalign}
where $\Phi_1$ is the potential of the solid, $\Phi_2$ is the potential of electrolyte, $U$ is the half-cell open circuit potential. The $V_{f,i}^*(x,t)=\mathit{ASR}_{f,i}^*Fj_i^*(x,t)$ is the voltage drop due to the film resistance, where $\mathit{ASR}_f$ is the area specific resistance. The modified current balance is as follows
\begin{flalign}
\label{curbal1}
\begin{cases}
\nabla~.~ i_2(x,t) = \sum_{i=1}^{N_n^R}a_i^nFj_i^n(x,t) & 0\le x<l_n,\\
\nabla~.~ i_2(x,t) =0 & l_n\le x\le l_n+l_s ,\\
\nabla~.~ i_2(x,t) = \sum_{i=1}^{N_p^R}a_i^pFj_i^p(x,t) & l_n+l_s<x\le l_{c},\\
\end{cases}
\end{flalign}
where $i_2$ is the current density in the electrolyte, the $a_i$ is the active interfacial surface area of particle $(i)$ per electrode unit volume, and the $l_{c}=l_n+l_s+l_p$ is denoting the total length of the cell. The boundary conditions are the continuity of $i_2$, and $i_2(0,t)=i_2(l_{c},t)=0$.
The following equations remain unchanged from the DFN model. The electrolyte material balance is
\begin{flalign}
\label{elecbal1}
\epsilon_2^{**} \frac{\partial c_{e}}{\partial t}(x,t)=\nabla~.~ (D_e^{eff} \nabla c_e(x,t))\\
+\frac{1-t_+^0}{F}\nabla~.~ i_2(x,t)-\frac{i_2~.~\nabla t_+^0 }{F}(x,t),
\end{flalign}
where the symbol $(**)$ can be $(p)$, $(n)$, and $(s)$ for positive electrode, negative electrode, and separator regions, $\epsilon_2$ is the porosity, $t_+^0$ is the transference number of Li ions, and the $D_e^{eff}=D_e(\epsilon_2^{**})^{brug}$ is the effective electrolyte diffusion coefficient. The boundary conditions are continuity of $c_{e}$, and $\nabla c_e(0,t)=\nabla c_e(l_{c},t)=0$. The liquid-phase Ohm's law is
\begin{flalign}
\label{liqOhm1}
i_2(x,t) = -\kappa^{eff}\nabla \Phi_2(x,t) + \frac{2\kappa^{eff}RT}{F}(1-t_+^0)\left( 1+\frac{d~ln~f_{\pm}}{d~ln~c_e}(x,t)  \right)\nabla (ln~c_e) (x,t),
\end{flalign}
where $f_{\pm}$ is the mean molar activity coefficient in the electrolyte, and the $\kappa^{eff}=\kappa(\epsilon_2^{**})^{brug}$ is the effective bulk ionic  conductivity of the electrolyte. The boundary conditions are continuity of $\Phi_2$, and $\Phi_2(0,t)=0$.
The solid-phase Ohm's law is
\begin{flalign}
\label{solOhm1}
i_1(x,t) = -\sigma^{eff} \nabla \Phi_1(x,t),
\end{flalign}
where $i_1$ is the current density in the solid, and the $\sigma^{eff}=\sigma(1-\epsilon_2^{*})^{brug}$ is the effective electronic conductivity. Also, $i_1(x,t)+i_2(x,t)=I(t)$, where $I(t)$ is the current density input to the model. Finally, the output of the model, voltage, is written as follows:
\begin{flalign}
\label{termVolt1}
V(t) = \Phi_1(l_{c},t)-\Phi_1(0,t).
\end{flalign}
Finally, the energy balance for the lithium ion battery assuming local thermal equilibrium is given by the following equations
%\begin{flalign}
%\label{energy1}
%\rho C_p \frac{dT}{dt}(t)-\dot{Q}=-\int_0^{l_n+l_s+l_p}\sum_{i=1}^{N_*}a_i^*j_i^*(x,t)U_{H,i}^*(x,t)dx+I(t)V(t),\\
%U_{H,i}^*(x,t)= U_*(c_{se,i}(x,t))-T(t)\frac{\partial U_*}{\partial T}(c_{se,i}(x,t)),
%\end{flalign}
\begin{flalign}
\label{energy1}
\frac{\partial (\rho C_p T)}{\partial t}=\nabla~.~(\lambda \nabla T)+q,
\end{flalign}
where $\rho$ is the volume average density, $C_p$ is the volume averaged specific heat, $T$ is the temperature, and $\lambda$ is the volume averaged thermal conductivity. The heat generation term, $q$, is given by
\begin{flalign}
\label{energy2}
q = \sum_{i=1}^{N_*}a_i^*Fj_i^*(x,t)\left(\eta_i^*(x,t)+T(t)\frac{\partial U_*}{\partial T}(c_{se,i}(x,t)) \right)-i_1\nabla \Phi_1 (x,t)- i_2\nabla \Phi_2 (x,t).
\end{flalign}
It is worth mentioning that this form neglects the enthalpy of mixing, since it is generally small and ignored in practice. Furthermore, the boundary conditions are defined based on the types of heat flux considered at the cell boundary such as, convection, conduction, and radiation.
\subsubsection{Reduced order model}
%The DFN model is pseudo 2 dimensional model, hence, it has its own fundamental assumption when it comes to modeling Lithium-ion batteries. However, the computation cost of this model is still high for estimation and control purposes. As a result, number of studies have emerged that using simplifying assumption to strike a balance between model accuracy and computation cost. 
For deriving the reduced order model, the asymptotic analysis method has been shown to result in a more accurate approximation of the full-order model compared to similar models in the literature \cite{marquis2019asymptotic}. Furthermore, this method requires no assumptions about the spatial distributions of variables. Using the same methodology, the resulting equations of the multi-particle model with electrolyte (MPMe) are presented in the following.

The behavior of all particles in each electrode can be represented by a single representative particle, with concentration $(c_{s,i})$
%Using the SPM assumption that Lithium concentrations, $(c_{s,i})$, and molar flux, $j_i$, are independent of space, the solid diffusion equations for each particle become
\begin{flalign}
\label{diff2}
\frac{\partial c_{s,i}^*}{\partial t}(r,t)=\frac{1}{r^2}\frac{1}{\partial r}\left[D_i^*r^2\frac{\partial c_{s,i}^*}{\partial r}(r,t)\right],\\
\frac{\partial c_{s,i}^*}{\partial r}(0,t)=0,\\
D_i^*\frac{\partial c_{s,i}^*}{\partial r}(R_{p,i}^*,t)=-j_i^*(t).
\end{flalign}
\par
Furthermore, for simplification it is assumed that the solid diffusion is independent of the concentration. The current exchange density, $i_0$, is approximated by integration over the electrode thickness, which results in the following for the Butler-Volmer equations
\begin{flalign}
\label{bv1}
j_i^*(t) = \frac{i_{0,i}^*(t)}{F}\left(e^{\frac{\alpha_a F}{RT}\eta_i^*}-e^{\frac{-\alpha_c F}{RT}\eta_i^*}\right), \\   
i_{0,i}^n(t) = \frac{1}{l_n} \int_{0}^{l_n} k_{0}^n(c_e(x,t))^{\alpha_a}(c_{s,max,i}^n-c_{se,i}^n(t))^{\alpha_a}(c_{se,i}^n(t))^{\alpha_c} dx, \\
i_{0,i}^p(t) = \frac{1}{l_p} \int_{l_c-l_p}^{l_c} k_{0}^p(c_e(x,t))^{\alpha_a}(c_{s,max,i}^p-c_{se,i}^p(t))^{\alpha_a}(c_{se,i}^p(t))^{\alpha_c} dx.
\end{flalign}
Observing that the total number of lithium moles are conserved in the solid and the electrolyte. This results in a simplified form for the current density in the electrolyte \cite{marquis2019asymptotic}, given by the following 
\begin{flalign}
\label{i2disturb}
\begin{cases}
 i_2(x,t) = \frac{I(t)}{l_n}x & 0\le x<l_n,\\
i_2(x,t) =I(t) & l_n\le x\le l_n+l_s ,\\
i_2(x,t) = -\frac{I(t)}{l_p}(x-l_{c})& l_n+l_s<x\le l_{c},\\
\end{cases}
\end{flalign}
Therefor using \cref{curbal1} results in
\begin{flalign}
I = \sum_{i=1}^{N_n^R}l_n a_{s,i}^n Fj_{i}^n, ~~ I = -\sum_{i=1}^{N_p^R} l_{p}a_{s,i}^p Fj_{i}^p.
\label{ch1}
\end{flalign}
Because of the conservation of lithium in the electrolyte the average lithium concentration over the cell length is equal to the initial concentration. Therefore, for the electrolyte concentration, an average transference number and diffusion coefficient based on electrolyte initial concentration is considered. The resulting equation when combining with \cref{ch1} is
\begin{flalign}
\label{elecconc3}
\epsilon_2^{**} \frac{\partial c_{e}}{\partial t}(x,t)=\nabla.(\bar{D_e}(\epsilon_2^{**})^{brugg} \nabla c_e(x,t))+\frac{1-\bar{t}_+^0}{F}\times
\begin{cases}
\frac{I(t)}{l_n} & 0\le x<l_n,\\
0 & l_n\le x\le l_n+l_s ,\\
\frac{-I(t)}{l_p} & l_n+l_s<x\le l_{c},\\
\end{cases}
\end{flalign}
where $\bar{t}_+^0=t_+^0(c_{e}^0)$ and $\bar{D_e} = D_e(c_{e}^0)$ with the same boundary conditions as the ones for \cref{elecbal1}. Similarly for solving the liquid-phase Ohm's law, \cref{liqOhm1}, the conductivity, $\kappa$, and the thermodynamic factor, $tf=(1-t_+^0)\left( 1+\frac{d~ln~f_{\pm}}{d~ln~c_e}(x,t)  \right)$ are calculated based on the average(initial) electrolyte concentration. Integrating and applying the boundary condition results in
\begin{flalign}
\Delta \Phi_2(t)= - \left( \frac{l_n}{3(\epsilon^n)^{brugg}}+ \frac{l_s}{(\epsilon^s)^{brugg}} +\frac{l_p}{3(\epsilon^p)^{brugg}}\right)\frac{I(t)}{\bar{\kappa}}+\frac{2RT}{Fc_{e,init}}\bar{tf}(\bar{c}_{e,p}-\bar{c}_{e,n}),
\label{electvolt2}
\end{flalign}
where $\bar{c}_{e,*}$ denotes the average electrolyte concentration over the electrode, the $\bar{\kappa} = \kappa(c_{e}^0)$, and  $\bar{tf} = tf(c_{e}^0)$. The solid electrical conductivity is large in the electrodes, which means the ohmic potential drop in the solid is relatively small, and the solid electric potential is independent of $x$. Hence, the solid-phase potential drop is negligible, and all the particles in an electrode have the same solid-phase potential and are essentially in a parallel configuration. This results in the following $(N_n^R-1)$ and $(N_p^R-1)$ equality equations for negative and positive electrodes, respectively, 
\begin{flalign}
\label{v1} 
\Phi_{1,1}^*=\Phi_{1,2}^*=...=\Phi_{1,N_*}^*.
\end{flalign}
Because of the above equations, the output voltage can be written for any index $i=1,...,N_p^R$ and $j=1,...,N_n^R$, therefore
 \begin{flalign}
\label{finalvt} 
V(t)=\eta_i^p(t)+U_p(c_{se,i}^p(t))+V_{f,i}^p(t)-\eta_j^n(t)-U_n(c_{se,j}^n(t))-V_{f,j}^n(t)+\Delta \Phi_2(t).
\end{flalign}

As for the energy balance equation, a lumped temperature model is considered, which reduces the complexity of the model. Furthermore, since the thickness of the cell is much smaller than the length scale for the heat conduction, the cell dissipates heat only through convection. With these assumptions the energy balance in reduced form is given by
\begin{flalign}
\label{energy1s}
\rho C_p \frac{dT}{dt}(t) =-\frac{hA_c(T(t)-T_{a})}{V_c}+\frac{1}{V_c}\int_{V_c}qd\nu,
\end{flalign}
where $h$ is the heat transfer coefficient for convection, $A_c$ is the battery surface area, $V_c$ is the cell volume, and $T_a$ is the ambient temperature. \cref{eta1} is used to substitute the over potential term, $\eta$, in \cref{energy2}, and further simplification of the above equation is done using the procedure in \cite{gu2000thermal}. Finally, the energy balance equation reduces to
\begin{flalign}
\label{energy2s}
\rho C_p l_c \frac{dT}{dt}(t)=-h(T(t)-T_{a})-\sum_{*=p\& n} \sum_{i=1}^{N_*^R}a_i^*Fj_i^*(t)l_*\left(U_*(c_{se,i}^*(t))+V_{f,i}^*(t)-T(t)\frac{\partial U_*}{\partial T}(c_{se,i}(t)) \right) -I(t)V(t).
\end{flalign}
\subsection{Mechanical Model}
In this section a model for the expansion of the lithium ion battery during cycling is presented. The model is developed by incorporating several simplifying assumptions. In our model, the expansion model does not affect the electrochemical model. It has been shown that for cells with a relatively small expansion such as graphite/NMC cell with 8 and 2$\%$ expansion of the anode and cathode respectively, the effect of stress induced diffusion in the solid for the voltage are negligible \cite{christensen2010modeling}. Additionally, an analysis of fundamental dimensionless parameters of a porous electrode model with the volume changes has shown that the dimensionless pressure parameter is orders of magnitude smaller than the other parameters \cite{sulzer2019faster}. Furthermore, adding the stress diffusion increases the complexity of the model substantially. Therefore, the effects of stress induced diffusion and volume changes on the terminal voltage are not considered. To further elucidate the model structure the coupling between the sub-models is shown in \cref{fig:diag}. 
\begin{figure}[!t]
	\centering
	{\includegraphics[width=0.5\columnwidth,trim = 0in 0in 0.0in 0in,clip=true]{figures/Flowchart.pdf}}
	\caption{Block diagram of the MPMe with expansion. Note that the coupling between the expansion subsystems and the electrochemical subsystem is one way.}
	\label{fig:diag}
\end{figure}
 \subsubsection{Intercalation induced expansion}
With the relatively small expansion of the cell, it is appropriate to utilize the infinitesimal strain theory for modeling the deformation. Thus the Cauchy strain tensor, $\bm{\epsilon}$, is given by
\begin{flalign}
{\bm{\epsilon}}=\frac{1}{2}\left(\nabla \bm{u} + (\nabla \bm{u})^T \right),
\label{Lag}
\end{flalign}
where $\bm{u}$ is displacement vector. The quasi-static condition is also assumed for the evolution of strain in the particle. With body forces neglected, the equilibrium condition reads as
\begin{flalign}
\nabla~.~\bm{\sigma}=0,
\label{equlib}
\end{flalign}
where $\bm{\sigma}$ is the Cauchy stress tensor. Furthermore, it is assumed that the bulk electrode particle is a linear elastic solid. The graphite material used in lithium-ion batteries is the mesophase carbon microbeads (MCMB), which is generally disordered, and thus it is assumed to be isotropic. The constitutive equations written using Young's modulus, $E$, and Poisson's ratio, $\nu$, are given by
\begin{flalign}
\epsilon_{ij}=\frac{1}{E}[(1+\nu)\sigma_{ij}-\nu \sigma_{kk}\delta_{ij}],
\label{d1}
\end{flalign}
where the equations are expressed with respect to a Cartesian coordinate system (e.g. $i,j,k=r,\theta,\phi)$, and the Einstein summation convention of summing on repeated indices is used. 
\par
During cycling the intercalation of lithium leads to changes in the lattice parameters. These changes can be represented as a volume change of some unit lattice volume, which in a macroscopic scale, is a function of the local lithium concentration. This change is represented by a volumetric strain, which is denoted by $\Delta \mathcal{V}$. Because of the assumptions of linear elasticity and small strain, this volumetric strain can be added to \cref{d1} linearly. This is equivalent to the treatment of the stress and strain induced by thermal expansion, first presented in \cite{prussin1961generation}, and in agreement with other studies \cite{christensen2010modeling,yang2005interaction,rieger2016new,zhang2007numerical}. Furthermore, the volumetric strain is equal in all direction, and hence it is trivial to show that the strain in the normal stresses direction is one third of the volumetric strain. Thus, the stress-strain relationship with intercalation expansion is given by
\begin{flalign}
\epsilon_{ij}=\frac{1}{E}[(1+\nu)\sigma_{ij}-\nu \sigma_{kk}\delta_{ij}]+\frac{\Delta \mathcal{V}\left(c_{s}(r,t)\right)}{3}\delta_{ij},
\label{d2}
\end{flalign}
where $\delta_{ij}$ is the Kronecker delta. It is assumed that the every active material particle is sphere, so a spherical coordinate system is utilized. Furthermore, due to the symmetry $\sigma_{\theta \theta}=\sigma_{\phi \phi}$, the normal strains in \cref{d2} can be written as
\begin{flalign}
\label{d23}
\epsilon_{rr}=\frac{1}{E}[\sigma_{rr}-2\nu \sigma_{\theta \theta}]+\frac{\Delta \mathcal{V}\left(c_{s}(r,t)\right)}{3}\\
\epsilon_{\theta \theta}=\frac{1}{E}[(1-\nu)\sigma_{\theta \theta}-\nu \sigma_{rr}]+\frac{\Delta \mathcal{V}\left(c_{s}(r,t)\right)}{3}
\label{d24}
\end{flalign}
The spherical symmetry of the particle also results in the radial and tangential stresses which are only a function of radial position. Therefore, the stress equilibrium equation (see \cref{equlib}) in the radial direction simplifies to
\begin{flalign}
\frac{\partial \sigma_{rr}}{\partial r}+\frac{2 (\sigma_{rr}-\sigma_{\theta \theta})}{r}=0,
\label{equlib2}
\end{flalign}
and the strain tensor equations (see \cref{Lag}) in spherical coordinates are
\begin{flalign}
\label{d3}
\epsilon_{rr}=\frac{\partial u_r}{\partial r}\\
\epsilon_{\theta \theta}=\frac{u_r}{r}
\label{d4}
\end{flalign}
where $u_r$ denotes radial displacement. Based on \cref{d23,d24,equlib2,d3,d4}, a second order differential equation for the radial displacement is obtained:
\begin{flalign}
\frac{\partial^2 u_r}{\partial r^2}+\frac{2}{r}\frac{\partial u_r}{\partial r}-\frac{2u_r}{r^2}=\frac{1+\nu}{1-\nu}\frac{\partial}{\partial r}\left(\frac{\Delta \mathcal{V}\left(c_{s}(r,t)\right)}{3}\right).
\label{diffu}
\end{flalign}
The boundary conditions are the displacement at the center being zero, and the stresses at the surface of particle being zero,
\begin{flalign}
u_r(0,t) = 0,\\
\sigma_{rr}(R_p,t) = 0.
\label{boundu}
\end{flalign}
Integrating \cref{diffu} along the radius of the particle subject to the two boundary conditions gives the solution for $u_r$,
\begin{flalign}
u_r(r,t)=\left[\frac{1+\nu}{1-\nu}\frac{1}{3r^2}+\frac{2(1-2\nu)}{1-\nu}\frac{r}{3R_{p}^3}\right]\int_0^{r} \rho ^2 \Delta \mathcal{V}\left(c_{s}(\rho,t)\right)d\rho.
\label{usol}
\end{flalign}
Finally, the displacement at the surface of the particle is calculated using \cref{usol} at $r = R_p$, which is the following,
\begin{flalign}
u_R(t)=\frac{1}{R_{p}^2}\int_0^{R_{p}} \rho ^2 \Delta \mathcal{V}\left(c_{s}(\rho,t)\right)d\rho.
\label{usol2}
\end{flalign}
\subsubsection{Electrode level expansion}
The electrode consists of active material, binder, and conductive material. The particle expansion results in deformation of the other components. In addition, the mechanical boundary conditions also impact the expansion. The electrode is fixed at the one side to the current collector and free on the separator side. In order to simplify the modeling of electrode expansion, the volume changes in other components is assumed to be negligible. Hence, the volume change of the electrode is given by
%\begin{flalign}
%\frac{\Delta V_e^*}{V_e^*}=\sum_{i=1}^{N_*^R}a_{i}^*u_{R,i}^*,
%\label{Eq:del-v}
%\end{flalign}
\begin{flalign}
\Delta V_e^*=\sum_{i=1}^{N_*^R}p_{i}^*\left(4\pi {R_{p,i}^*}^2 \right) u_{R,i}^*,
\label{Eq:del-v}
\end{flalign}
where $p_i$ is the total number of particles with a radius $R_{p,i}$ in the electrode. Furthermore, because of the large electrode length to thickness ratio and high stiffness, it is assumed that the electrode only expands in the through-plane direction \cite{rieger2016strain}. Therefore, the volume change can also be written as
\begin{flalign}
\Delta V_e^* = A\Delta t_*.
\label{Eq:del-t1}
\end{flalign}
Following the definition of $a^*_i$, which is the active interfacial surface area of particles with size $R_{p,i}^*$ per unit volume of the electrode, we have:
\begin{flalign}
a^*_i = \frac{p_{i}^*\left(4\pi {R_{p,i}^*}^2 \right) }{Al_*}.
\label{Eq:del-t2}
\end{flalign}
Using \cref{Eq:del-v,Eq:del-t1,Eq:del-t2} together results in the following equation for the change in electrode thickness,
\begin{flalign}
\Delta t_*=\sum_{i=1}^{N_*^R}a_{i}^*u_{R,i}^*l_*.
\label{Eq:del-t3}
\end{flalign}

\begin{figure}[!t]
	\centering
	{\includegraphics[width=\columnwidth,trim = 0in 2.0in 0.0in 0in,clip=true]{figures/sls_3.pdf}}
	\caption{a) The fixture schematics, and b) the simplified linear spring model for the battery.}
	\label{fig:sls}
\end{figure}

\subsubsection{Thermal and battery level expansion}
Since it was assumed that the temperature is uniform in the cell, a lumped expansion model is also considered for the battery. Therefore, the thermal expansion, $\Delta t_{th}$, is given by
\begin{flalign}
\Delta t_{th}=\alpha_{th}(T-T_{a}),
\label{Eq:del-th}
\end{flalign}
where $\alpha_{th}$ is the thermal expansion coefficient of the battery. The total expansion of the electrodes in the cell is simply the sum of the expansion of individual electrodes. Furthermore, in the case of this paper, the battery consists of multiple layers of cells stacked on top of each other in a pouch cell. Hence, the total expansion of electrodes is given by
\begin{flalign}
\Delta t_e = n_c\left(\Delta t_p+\Delta t_n\right),
 \label{eq:delt-t-c}
\end{flalign}
where $n_c$ is the number of parallel cells stacked on top of each other in the battery. However, for the expansion at the battery level it is also necessary to consider the influence of the inactive components such as the separator, current collectors, and casing. The expansion and the strain rate during battery cycling is small enough to consider a linearized regime for the deformation of these components. Furthermore, the assumption of quasi-equilibrium is considered. Therefore, the modeling of the inactive components is achieved with a linear spring in series with the electrodes. Additionally, a linear spring is also considered to account for the effects of the fixture on the expansion. The configuration of the spring model is shown in \cref{fig:sls}(b). As the amount of force is the same in the springs, following equation can be written for the expansion at the battery level
\begin{flalign}
\Delta t_b = \kappa_b \Delta t_e,
 \label{eq:delt-t-b}
\end{flalign}
where $\kappa_b=\frac{k_{ic}}{k_{ic}+k_f}$ with $k_{ic}$ and $k_f$ denoting the inactive components and fixture spring constants, respectively. Finally,
\begin{flalign}
\delta = \Delta t_b+\Delta t_{th}.
 \label{eq:delt-t-tot}
\end{flalign}
where $\delta$ denotes the total expansion of the battery.

==> Extra/packages.tex <==
\usepackage{array, threeparttable, booktabs, caption} % commands for table rules
\usepackage{multirow}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\usepackage{etoolbox}
\makeatletter
\patchcmd{\@makecaption}
  {\scshape}
  {}
  {}
  {}
\makeatother

==> Extra/rough.tex <==
%\title{Enhancing State Estimation in a Li-ion Battery using Expansion}
% \title{Application of Expansion for Enhancing State Estimation of a Electrochemical Battery System}
% \author{
% \IEEEauthorblockN{Sravan Pannala}
% \IEEEauthorblockA{\textit{Mechanical Engineering} \\
% \textit{University of Michigan}\\
% Ann Arbor, USA \\
% spannala@umich.edu}

% \and
% \IEEEauthorblockN{Puneet Valecha}
% \IEEEauthorblockA{\textit{Powertrain OBD Calibration} \\
% \textit{Fiat Chrysler Automotive}\\
% Chelsea, USA \\
% valechap@umich.edu}

% \and
% \IEEEauthorblockN{Peyman Mohtat}
% \IEEEauthorblockA{\textit{Mechanical Engineering} \\
% \textit{University of Michigan}\\
% 		Ann Arbor, USA \\
% 		pmohtat@umich.edu}
% \and
% \IEEEauthorblockN{Jason B. Siegel}
% \IEEEauthorblockA{\textit{Mechanical Engineering} \\
% \textit{University of Michigan}\\
% 		Ann Arbor, USA \\
% 		sigeljb@umich.edu}
% \and
% \IEEEauthorblockN{Anna G. Stefanopoulou}
% \IEEEauthorblockA{\textit{Mechanical Engineering} \\
% \textit{University of Michigan}\\
% 		Ann Arbor, USA \\
% 		annastef@umich.edu}

% }


% \begin{figure*} [h]
% 	\centering
% 	\subfigure[Current]{\includegraphics[width=0.45\linewidth]{figures/s1_cur.png}}
%     \subfigure[Voltage]{\includegraphics[width=0.45\linewidth]{figures/s1_vol.png}}
%     \subfigure[Expansion]{\includegraphics[width=0.45\linewidth]{figures/s1_exp.png}}
%     \subfigure[Voltage and Exp Error]{\includegraphics[width=0.45\linewidth]{figures/s1_err.png}}
%     \subfigure[$c_s^-$]{\includegraphics[width=0.45\linewidth]{figures/s1_anconc.png}}
%     \subfigure[$c_s^+$]{\includegraphics[width=0.45\linewidth]{figures/s1_caconc.png}}
% 	\caption{Constant Current}
% 	\label{fig:sim1}
% \end{figure*}

% \begin{figure*} [h]
% 	\centering
% 	\subfigure[Current]{\includegraphics[width=0.45\linewidth]{figures/s2_cur.png}}
%     \subfigure[Voltage]{\includegraphics[width=0.45\linewidth]{figures/s2_vol.png}}
%     \subfigure[Expansion]{\includegraphics[width=0.45\linewidth]{figures/s2_exp.png}}
%     \subfigure[Voltage and Exp Error]{\includegraphics[width=0.45\linewidth]{figures/s2_err.png}}
%     \subfigure[$c_s^-$]{\includegraphics[width=0.45\linewidth]{figures/s2_anconc.png}}
%     \subfigure[$c_s^+$]{\includegraphics[width=0.45\linewidth]{figures/s2_caconc.png}}
% 	\caption{Drive Cycle}
% 	\label{fig:sim2}
% \end{figure*}


The stress strain relationship in the particle with intercalation expansion is given by \cref{eq:stress_strain_1,eq:stress_strain_2}, the stress equilibrium in radial direction is given by \cref{eq:stress_eqb} and the strain displacement relationship is given by \cref{eq:strain_disp_1,eq:strain_disp_2}, where $\mathcal{V}({c}_s(r))$ is the volumetric strain function also reffered to as expansion function in this paper and $u_r$ is the radial displacement. 
\begin{flalign}
\label{eq:stress_strain_1}
\epsilon_r=\frac{1}{E}\left[\sigma_r-2\nu\sigma_t\right]+\frac{\Delta\mathcal{V}\left({c}_s(r)\right)}{3}\\
\label{eq:stress_strain_2}
\epsilon_t=\frac{1}{E}\left[{\left(1-\nu\right)\sigma}_t-\nu\sigma_r\right]\frac{\Delta\mathcal{V}\left({c}_s(r)\right)}{3}\\
\label{eq:stress_eqb}
\frac{d\sigma_r}{dr}+\frac{2\left(\sigma_r-\sigma_t\right)}{r}=0\\
\label{eq:strain_disp_1}
\epsilon_r=\frac{du_r}{dr}\\
\label{eq:strain_disp_2}
\epsilon_t=\frac{u_r}{r}
\end{flalign}
Using \cref{eq:stress_strain_1,eq:stress_strain_2,eq:stress_eqb,eq:strain_disp_1,eq:strain_disp_2}, we obtain a differential equation for $u_r$ as shown in \cref{eq:displ_diff}.
\begin{flalign}
\label{eq:displ_diff}
\frac{d^2u_r}{dr^2}+\frac{2}{r}\frac{du_r}{dr}- \frac{2u_r}{r^2}=\frac{1+\nu}{1-\nu}\frac{d}{dr}\left(\frac{\Delta\mathcal{V}\left({c}_s(r)\right)}{3}\right)\\
\label{eq:displ_bc_1}
u_r\left(0,t\right)=0\\
\label{eq:displ_bc_2}
\sigma_r\left(R_p,t\right)=0
\end{flalign}
 The displacement at the surface of the particle is obtained by solving \cref{eq:displ_diff} with the boundary conditions \cref{eq:displ_bc_1,eq:displ_bc_2} and is given by \cref{eq:ur}.
 \begin{flalign}
\label{eq:ur}
u_R(t)=\frac{1}{(R_{p})^2}\int_0^{R_{p}} \rho ^2 \Delta \mathcal{V}\left(c_s(\rho,t)\right)d\rho\\
\end{flalign}

\begin{table}[!t]\centering
\ra{0.9}
\scriptsize
\begin{tabular}{p{4cm}p{3cm}}\toprule
{Pouch cell} & \\ \midrule
{Nominal capacity} & \multicolumn{1}{r}{5.0 Ah}\\
{Operating voltage} & \multicolumn{1}{r}{3.0-4.2 V}\\ 
{Thickness} & \multicolumn{1}{r}{4.0 mm}\\ 
{Length} & \multicolumn{1}{r}{132 mm}\\ 
{Width} & \multicolumn{1}{r}{90 mm}\\ \\
Positive electrode \\ \midrule
Material & \multicolumn{1}{r}{NMC111:CB:PVDF (94:3:3)}\\
\\
Negative electrode \\ \midrule
Material & \multicolumn{1}{r}{Graphite:PVDF (95:5)}\\
\\ 
Separator \\ \midrule
Material & \multicolumn{1}{r}{Polyethylene (PE)}\\ \\
Electrolyte \\ \midrule
Material & \multicolumn{1}{r}{1 M $LiPF_6$}\\ 
Organic solvent in electrolyte & \multicolumn{1}{r}{$2\%$ EC:EMC (3:7)}\\ \bottomrule
\end{tabular}
\caption{The pouch cell specifications.}
\label{tabel1}
\end{table}
